Partial Distribution Matching via Partial Wasserstein Adversarial Networks

This paper studies the problem of distribution matching (DM), which is a fundamental machine learning problem seeking to robustly align two probability distributions. Our approach is established on a relaxed formulation, called partial distribution matching (PDM), which seeks to match a fraction of the distributions instead of matching them completely. We theoretically derive the Kantorovich-Rubinstein duality for the partial Wasserstain-1 (PW) discrepancy, and develop a partial Wasserstein adversarial network (PWAN) that efficiently approximates the PW discrepancy based on this dual form. Partial matching can then be achieved by optimizing the network using gradient descent. Two practical tasks, point set registration and partial domain adaptation are investigated, where the goals are to partially match distributions in 3D space and high-dimensional feature space respectively. The experiment results confirm that the proposed PWAN effectively produces highly robust matching results, performing better or on par with the state-of-the-art methods.

==> tex_file/bio.tex <==
\vskip -1.6\baselineskip plus -1fil


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{tex_file/ZMW}}]{Zi-Ming Wang}
	received his Ph.D degree in Computer vision from Wuhan University, Wuhan, China, in 2022. 
  He is currently working as a postdoc in Chalmers University in Gothenburg, Sweden. 
  His research interests include generative models and point cloud processing.
\end{IEEEbiography}

\vspace{-2mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.in,clip,keepaspectratio]{tex_file/nxue2.png}}]{Nan Xue}(Member, IEEE) is currently a research scientist at Ant Research, affiliated with Ant Group. Previously, from 2020 to 2023, he served as a research associate professor in the School of Computer Science at Wuhan University. He earned his Ph.D. degree in 2020 and B.S. degree in 2014, both from Wuhan University. From 2018 to 2020, he worked as a visiting Ph.D. student with the iVMCL Group at NC State University. He is a recepient of the Outstanding Doctoral Dissertation Award, by China Society of Images and Graphics in 2022. His current research interest is around the Structured Visual Geometry in 2D and 3D vision.
\end{IEEEbiography}

\vspace{-2mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{tex_file/Leiling}}]{Ling Lei}
received her B.Sc. and M.Sc. degree from Central China Normal University in 2001 and 2004 respectively, and Ph.D. degree from Zhejiang University in 2007. She is currently working as an Associate Professor in the School of Mathematics and Statistics, Wuhan University. Her research interests include optimal control theory and computer vision.
\end{IEEEbiography}

\vspace{-2mm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{tex_file/RJornsten_jpg}}]{Rebecka Jörnsten}
received her M.Sc. in Engineering Physics from Lund Institute of Technology (LTH) 
in 1991 and her Ph.D. in Statistics from the University of California at Berkeley in 2001. 
She is currently a Professor of Applied Statistics and Biostatistics at the Department of 
Mathematical Sciences, University of Gothenburg/Chalmers University of Technology. 
From 2002 to 2008 she was an assistant and then associate Professor at Rutgers University. 
She joined the University of Gothenburg/Chalmers in 2009. Her research interests include
high-dimensional statistics, regularization and optimization in machine learning, and data integration.
\end{IEEEbiography}

\vspace{-2mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{tex_file/xgs-2024-google}}]{Gui-Song Xia}
(M'10-SM'15) received his Ph.D. degree in image processing and computer vision from CNRS LTCI, T{\'e}l{\'e}com Paris, Paris, France, in 2011. From 2011 to 2012, he has been a Post-Doctoral Researcher with the Centre de Recherche en Math{\'e}matiques de la Decision, CNRS, Paris-Dauphine University, Paris, for one and a half years.
He is currently a Hongyi Distinguished Professor at Wuhan University, leading a research group working on Computer Vision and Robotics. He has also been working as Visiting Scholar at DMA, {\'E}cole Normale Sup{\'e}rieure (ENS-Paris) for two months in 2018. His current research interests include computer vision, robotics and remote sensing imaging. 
He served/serves on the Editorial Boards of several journals, including {\em ISPRS Journal of Photogrammetry and Remote Sensing, Pattern Recognition, Signal Processing: Image Communications, EURASIP Journal on Image \& Video Processing, Journal of Remote Sensing, and Frontiers in Computer Science: Computer Vision}.
\end{IEEEbiography}


